TP3M: Transformer-based Pseudo 3D Image Matching with Reference Image

Image matching is still challenging in such scenes with large viewpoints or illumination changes or with low textures. In this paper, we propose a Transformer-based pseudo 3D image matching method. It upgrades the 2D features extracted from the source image to 3D features with the help of a reference image and matches to the 2D features extracted from the destination image by the coarse-to-fine 3D matching. Our key discovery is that by introducing the reference image, the source image's fine points are screened and furtherly their feature descriptors are enriched from 2D to 3D, which improves the match performance with the destination image. Experimental results on multiple datasets show that the proposed method achieves the state-of-the-art on the tasks of homography estimation, pose estimation and visual localization especially in challenging scenes.

==> figs/Fig4.tex <==
\begin{figure}[t]
    \centering
        \includegraphics[width=\linewidth]{images/4.png} 
    \caption{Pseudo 3D feature extraction consisting of 3D feature computing and fusion.}
    \label{fig:3D_Feature}
\end{figure}


==> figs/Fig5.tex <==
\begin{figure}[t]
    \centering
        \includegraphics[scale=0.35]{images/5.png} 
    \caption{Cross-attention layer in 3D feature matching. It matches 2D features and 3D features.}
    \label{fig:Cross-attention}
\end{figure}


==> figs/Fig6.tex <==
\begin{figure}[t]
    \centering
	\includegraphics[width=0.49\linewidth]{images/7_a.png} 
        \includegraphics[width=0.49\linewidth]{images/7_b.png}
	\includegraphics[width=0.49\linewidth]{images/7_c.png} 
        \includegraphics[width=0.49\linewidth]{images/7_d.png}
    \caption{Features distribution on Megadepth. Left: Matching features of Matchformer. Right: Matching features of TP3M, they are obviously distributed at the edge.}
    \label{fig:Features distribution}
\end{figure}


==> figs/Fig7.tex <==
\begin{figure*}[t]
    \centering
	\rotatebox{90}{{~~~~~~~\textbf{HPatches}}}~~
	\includegraphics[width=0.42\linewidth]{images/6_1a.png} 
	\includegraphics[width=0.42\linewidth]{images/6_1b.png} \\
	\rotatebox{90}{{~~~~~~~\textbf{ScanNet}}}~~
	\includegraphics[width=0.42\linewidth]{images/6_2a.png} 
	\includegraphics[width=0.42\linewidth]{images/6_2b.png} \\
	\rotatebox{90}{{~~~~~~~\textbf{MegaDepth}}}~
	\includegraphics[width=0.42\linewidth]{images/6_3a.png} 
	\includegraphics[width=0.42\linewidth]{images/6_3b.png} \\
	\rotatebox{90}{{~~~~~~~\textbf{Aachen}}}~~
	\includegraphics[width=0.42\linewidth]{images/6_4a.png} 
	\includegraphics[width=0.42\linewidth]{images/6_4b.png} \\
	\rotatebox{90}{{~~~~~~~\textbf{InLoc}}}~~
	\includegraphics[width=0.42\linewidth]{images/6_5a.png} 
	\includegraphics[width=0.42\linewidth]{images/6_5b.png}
	\rotatebox{0}{{\textbf{MatchFormer}~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\textbf{TP3M}}} 
    \caption{Qualitative results on challenging image pairs. MatchFormer do not capture enough correspondences in the pairs with large viewpoint change or illumination change. MatchFormer’s matches are less than TP3M’s especially in the pair of InLoc. TP3M establishes more accurate and robust matching at the edge.}
    \label{fig:Qualitative_results}
\end{figure*}


==> figs/Fig8_-_______.tex <==
\begin{figure}[t]
    \centering
        \includegraphics[width=0.31\linewidth]{images/8_a.jpeg} 
        \includegraphics[width=0.31\linewidth]{images/8_b.jpeg}
        \includegraphics[width=0.31\linewidth]{images/8_c.jpeg} \\
        \includegraphics[width=0.47\linewidth]{images/8_d.jpeg}
        \includegraphics[width=0.47\linewidth]{images/8_e.jpeg}
    \caption{Visualizing attention. Up: 2D self-attention in source image, 3D self-attention in source image, 2D self-attention in destination image. Down: 2D-2D and 2D-3D cross-attention between source and destination image.}
    \label{fig:Visualizing_attention}
\end{figure}

